Improved currents for $\bar{B}\to D^{(*)}\ell\bar{\nu}$ form factors from Oktay-Kronfeld heavy quarks

The CKM matrix element $|V_{cb}|$ can be extracted by combining experimentally determined branching fractions for $\bar{B}\to D^{(*)}\ell\bar{\nu}$ decays with form factors from the lattice. While successful, the precision of this approach has been limited by heavy-quark discretization effects. An improved version of the Fermilab action, the Oktay-Kronfeld action, can be used to reduce heavy-quark discretization effects in calculations performed at the physical bottom and charm quark masses. Treating charm and bottom quarks as massive, we are carrying out improvement of the flavor-changing currents through third order in the momentum (HQET) expansion.

==> Makefile <==
DRIVE = $(HOME)/Library/GoogleDrive/Tmp/

#---------------------------------------------------------------------

TEXS := $(wildcard *.tex tables/*.tex eqns/*.tex)
MAIN := main.tex

PDF_FIG := $(wildcard ./figs/*.pdf)

AUX = $(wildcard *.aux *.log *.nav *.out *.snm\
	             *.toc *.vrb *.bbl *.blg *.dvi\
				 *.lof *.lot)

TARGET = $(MAIN:%.tex=%.pdf)

#---------------------------------------------------------------------

LATEX := latex
PDFLATEX := pdflatex

#---------------------------------------------------------------------

all : $(TARGET) 
	make tmpclean

debug : $(TARGET)

cloud : build
	cp -a $(TARGET) $(DRIVE)

#tmpclean:
#	@rm -f $(AUX)

#clean:
#	@rm -f $(AUX) $(TARGET)

%.pdf : %.tex $(MAIN) $(TEXS) $(PDF_FIG) Makefile refs.bib
	$(PDFLATEX) $(basename $<)
	bibtex      $(basename $<)
	$(PDFLATEX) $(basename $<)
	$(PDFLATEX) $(basename $<)
	$(PDFLATEX) $(basename $<)



==> eqns/FF-h.tex <==
\begin{align}
F_D(\omega) &= h_+(\omega) + \left(\frac{1-r}{1+r}\right)h_-(\omega)\,,\\
F_{D^*}^2(\omega) &= \frac{ 1 }{ 12 (1 - r^*)^2 \chi(\omega) }\Biggl\{ \biggl[(\omega - r^*) ( \omega + 1 ) h_{A_1}(\omega) \\
&-\ (\omega^2 - 1) \left(r^*h_{A_2}(\omega) + h_{A_3}(\omega)\right) \biggr]^2 + 2 ( 1 - 2 \omega r^* + r^{*2} ) \\
&\times\ \left[ ( \omega + 1 )^2 h_{A_1}^2(\omega) + (\omega^2 - 1)h_V^2(\omega) \right] \Biggr\}\,.
\end{align}


==> eqns/dparams2.tex <==
\begin{align}
d_1 = \frac{\zeta}{2\sinh\,M_1} - \frac{1}{2m_q}\,,\quad\quad
d_2 = d_1^2 - \frac{r_s\zeta}{2e^{M_1}}\,,\quad\quad
d_B = d_1^2 - \frac{c_B\zeta}{2e^{M_1}}\,.
\end{align}


==> eqns/ff-hme.tex <==
\begin{align}
\frac{\matrixe{D(p_D)}{V^{\mu}}{B(p_B)}}{\sqrt{M_D M_B}} &= (v_B + v_D)^{\mu}h_+(\omega) + (v_B - v_D)^{\mu}h_-(\omega)\,,\\
\frac{\matrixe{D^*(p_{D^*},\bar{\epsilon})}{A^{\mu}}{B(p_B)}}{\sqrt{M_{D^*} M_B}} &= i\left[\bar{\epsilon}^{*\mu}(1 + \omega)h_{A_1}(\omega) - (\bar{\epsilon}^* \cdot v_B)\left(v_B^{\mu} h_{A_2}(\omega) + v_{D^*}^{\mu} h_{A_3}(\omega)\right)\right]\,,\\
\frac{\matrixe{D^*(p_{D^*},\bar{\epsilon})}{V^{\mu}}{B(p_B)}}{\sqrt{M_{D^*} M_B}} &= \varepsilon^{\mu\nu}_{\rho\sigma} \bar{\epsilon}^*_{\nu} v^{\rho}_B v^{\sigma}_{D^*} h_V(\omega)\,.
\end{align}

